Teapot: Efficiently Uncovering Spectre Gadgets in COTS Binaries

Speculative execution is crucial in enhancing modern processor performance but can introduce Spectre-type vulnerabilities that may leak sensitive information. Detecting Spectre gadgets from programs has been a research focus to enhance the analysis and understanding of Spectre attacks. However, one of the problems of existing approaches is that they rely on the presence of source code (or are impractical in terms of run-time performance and gadget detection ability). This paper presents Teapot, the first Spectre gadget scanner that works on COTS binaries with comparable performance to compiler-based alternatives. As its core principle, we introduce Speculation Shadows, a novel approach that separates the binary code for normal execution and speculation simulation in order to improve run-time efficiency. Teapot is based on static binary rewriting. It instruments the program to simulate the effects of speculative execution and also adds integrity checks to detect Spectre gadgets at run time. By leveraging fuzzing, Teapot succeeds in efficiently detecting Spectre gadgets. Evaluations show that Teapot outperforms both performance (more than 20x performant) and gadget detection ability than a previously proposed binary-based approach.

==> apdx-coverage.tex <==
\section{Code Coverage}


\begin{table}[t]
  \centering
  \caption{Maximum reached coverage of the evaluated real-world vanilla binary programs.}{
  \rowcolors{3}{gray90}{}
  \resizebox{0.45\textwidth}{!}{
    {\renewcommand{\arraystretch}{1.2}
    \begin{tabular}{c<{\hspace{1pc}} c c<{\hspace{1pc}} c c} %
      \toprule
      \multirow{2}{*}{Program} & SpecFuzz & SpecFuzz & \multicolumn{2}{c}{\toolname{} (Proposed)} \\
      & (Reported\cite{SpecFuzz}) & (Reproduced) & \normalfnname{} & \specfnname{} \\
      \midrule
      jsmn & 96.6\% & 98.89\% & 98.85\% & 84.71\% \\
      libyaml & 63.3\% & 68.93\% & 46.17\% & 72.08\% \\
      libhtp & 60.6\% & 61.43\% & 58.71\% & 54.09\% \\
      brotli & 84.1\% & 82.58\% & 82.54\% & 87.92\% \\
      openssl & 24.0\% & N/A & 20.86\% & 21.70\% \\
      \bottomrule
    \end{tabular}}\label{tab:exp-cov-v1}
  }
}
\end{table}

The maximum reached coverage of the real-world binaries tested in \cref{ssec:exp-fuzz-v1} is shown in \cref{tab:exp-cov-v1}.
Note that SpecFuzz did not report correct coverage information for \texttt{openssl} (0\% coverage was reported) on our test platform, so we leave it as unavailable.
We also do not report and compare coverage from SpecTaint as this information is not made public in their paper.
Smaller and simpler programs such as \texttt{jsmn} and \texttt{brotli} reached higher coverages.
In contrast, complex programs such as \texttt{openssl} show low code coverage, which is expected as it contains various fuzzing drivers that cover different parts of the program.
We can see that binaries instrumented by \toolname{} achieve comparable coverage between \normalfnname{} and \specfnname{}.
\toolname{} achieves lower coverage in the \normalfnname{} compared to SpecFuzz.
We believe this is due to \toolname{}'s nested speculation heuristics searching the \specfnname{} more extensively than SpecFuzz, which inevitably takes more time.


==> apdx-design-choices.tex <==
\section{Design Choices in \twocopyname{}}\label[appendix]{sec:apdx-design-choices}

\subsection{Difficulties of implementing \twocopyname{} in the compiler}
It may intuitively seem like \twocopyname{} is not specific to binary-level instrumentation and previous LLVM-based works\cite{SpecFuzz,Kasper} can benefit from applying a similar design.
For example, Split Kernel\cite{SplitKernel} features a design sharing some similarities with \twocopyname{} to achieve selective kernel hardening, and the proposed approach was successfully implemented on a compiler.
However, we consider implementing \twocopyname{} on compiler frontends very difficult.

The main reason for the difficulty is that LLVM IR strictly forbids basic block level control flow transitions out of the current function\cite{LLVMLangRef}.
This is a necessity for implementing \twocopyname{}.
It is also impossible to compile the source program twice with different instrumentation passes respectively and combine them: the two runs likely receive different optimizations, or at the very least, individual instructions will get varying register assignments, making them not interoperable at the basic block level.
In contrast, Split Kernel\cite{SplitKernel} only requires control flow transitions between functions, which is permitted and well defined by the calling conventions.

\twocopyname{} originates from the unique flexibilities of binary instrumentation, enabling performance optimizations beyond the capabilities of compiler-frontend-based solutions.
The run-time performance of the instrumented binaries is highly comparable with compiler-instrumented binaries, which we demonstrate further in \cref{ssec:exp-runtime-perf}.


\subsection{Handling indirect branches}

\begin{lstlisting}[style=my-lst-style-linenum, caption={An alternative design for handling indirect branches which is not suitable for \twocopyname{}. (Based on Listings 1 and 2 of Split Kernel\cite{SplitKernel}.)}, label={lst:apdx-ind-br-patch}, float=t, language={[x64]Assembler}]
.quad bar$hdn       ;pointer to hardened copy
bar:
  ; ...

foo$hdn:
  ; ...
  ; call rax        ;original indirect call
  mov rax, [rax-8]  ;fetch hardened copy pointer
  call rax          ;call hardened copy instead
  ; ...
\end{lstlisting}

We discuss one alternative design choice for handling returns and indirect calls/jumps that has been considered (and suggested by many), but was determined to be inappropriate for \twocopyname{} and thus not selected.
Split Kernel\cite{SplitKernel} proposed selective kernel hardening at the function granularity, and their design principles share some similarities with \twocopyname{}.
In their work, each kernel function is compiled twice with hardening on and off respectively, and the hardened copy is invoked only when necessary (decided at system call boundaries) to improve performance.

To prevent control flow from escaping into unhardened functions, Split Kernel proposes the design shown in \cref{lst:apdx-ind-br-patch}.
For each unhardened function, an inline pointer to the hardened copy is inserted before the function prologue (line~1).
Indirect calls in the hardened copy are transformed to fetch and call the hardened copy pointer instead (lines~8--9).
Admittedly, compared to the design featured in \twocopyname{} (\cref{ssec:twocopy-ind-call}), the overhead of this approach is lower, as only one extra pointer dereferencing is required.

However, the main difference between Split Kernel and \twocopyname{} is that Split Kernel guarantees the hardened mode is always entered and exited at system calls (as whether to use the hardened kernel is determined by the trustworthiness of the user-space program). 
Therefore, the indirect branch problem in that context is greatly simplified:
\begin{enumerate}
    \item There are no control flow transitions between the hardened and unhardened copy on the basic block level. Embedding data between functions is generally safe as there is no fallthrough execution.
    \item Since hardened functions' entry and exit points are fixed (only at the system calls), no return from the hardened function into unhardened parts of the kernel is possible. Therefore, this design should only consider indirect function calls to unhardened functions.
    \item As Split Kernel is implemented on the compiler, complete control flow information is available.
\end{enumerate}

The situation in \twocopyname{} is more complex as:
\begin{enumerate}
    \item Simulation may be entered from basic block boundaries, and it is impractical to insert \specfnname{} pointers as data between basic blocks: fallthrough execution happens, and extra care must be taken to skip the data from being executed as instructions.
    \item \specfnname{} functions may return out of the current function, and properly handling such cases is required.
    \item The discovery of all control flow paths is not guaranteed with binary disassemblers; thus, a safeguard (lines~8--9 of \cref{lst:ind-br-patch}) is required.
\end{enumerate}
Hence, we determined that the above limitations make the approach shown in \cref{lst:apdx-ind-br-patch} inappropriate for \twocopyname{}.


==> apdx-specfuzz.tex <==
\section{\toolname{}-SpecFuzz: an alternative \toolname{} implementation with SpecFuzz policies}\label[appendix]{sec:apdx-sf}
In \cref{ssec:motivations-compiler}, we brought attention to certain pitfalls within compiler-based analysis tools such as SpecFuzz\cite{SpecFuzz}, despite them being generally considered more effective than binary-based tools when source code is available. 
To demonstrate this point, we facilitate a more fine-grained comparison with SpecFuzz.
We present an alternative implementation of \toolname{} with the SpecFuzz gadget policies shown below, and we call this implementation \toolname{}-SpecFuzz.\footnote{Note that \toolname{}-SpecFuzz is subject to the same limitations of the SpecFuzz policy, including inevitably reporting more false positives. \toolname{} with the Kasper policies is more suitable for real-world usage.}

\fbox{
\begin{minipage}{0.9\linewidth}
  \textbf{SpecFuzz policy}: if an instruction \textit{transiently accesses out-of-bounds memory}, it is a gadget.
\end{minipage}
}

Except for the different gadget policy, \toolname{}-SpecFuzz is based on the same building blocks, including \twocopyname{}, and behaves mostly identically to \toolname{}.
However, a few implementation differences should be noted:
\begin{itemize}
    \item Binary DIFT functionalities (\cref{sssec:nahco3-dift}) are removed as they are not required by the SpecFuzz policy.
    \item We did not implement nested speculation support on \toolname{}-SpecFuzz. The following experiments are therefore conducted with nested speculation also disabled on SpecFuzz.
\end{itemize}

We conduct the experiments on the same set of binaries described in \cref{sec:experiments}.
Note that the following experiments are conducted on a different machine (two Intel Xeon E5-2680 v4, each 14C/28T, \SI{2.40}{\giga\hertz}, with \SI{192}{\giga\byte} of RAM), so the results are not directly comparable with the previous ones. 
We demonstrate replicas of the experiments described in \cref{ssec:exp-runtime-perf,ssec:exp-fuzz-v1}, namely the run-time performance and real-world binaries fuzzing experiments, to showcase the effectiveness of \toolname{}-SpecFuzz against SpecFuzz.
We finally case study a SpecFuzz-type gadget overlooked by the original SpecFuzz but discovered by \toolname{}-SpecFuzz.

With the above experiment setting, neither SpecFuzz nor \toolname{}-SpecFuzz detected any gadgets from \texttt{jsmn} (that are not protected by multiple nested branches), so we omit it from the following results.

\subsection{Run-time performance}\label[appendix]{ssec:apdx-expsf-runtime}
We compare the raw run-time performance of the instrumented programs with SpecFuzz and \toolname{}-SpecFuzz under similar experiment settings as in \cref{ssec:exp-runtime-perf}.
Note that nested speculation support is disabled for a fair comparison.

\input{figs/expsf-runtime-overhead}

The normalized execution time is shown in \cref{fig:expsf-runtime-overhead}.
Despite being fully binary-based, \toolname{}-SpecFuzz greatly outperforms the original SpecFuzz implementation (2.5$\times$ on average).
This is different from what we observed in \cref{ssec:exp-runtime-perf} with SpecFuzz and \toolname{} with Kasper policies.
The original \toolname{} is inevitably a heavier implementation because of the complexity of Kasper policies (especially with the requirement of Binary DIFT).
The performance gain of \toolname{}-SpecFuzz compared to the original SpecFuzz more clearly showcases the superiority of \twocopyname{}.
We mainly attribute this performance difference to the fact that SpecFuzz needs to check the current program mode before executing every single instrumentation code because normal and speculative mode codes are mixed together; in addition, SpecFuzz relies on the LLVM frontend to generate ASan instrumentation, which is always executed regardless of the run-time mode.

\subsection{Fuzzing unmodified real-world binaries}\label[appendix]{ssec:apdx-expsf-fuzz}
\begin{table}[t]
  \centering
  \caption{Maximum reached coverage of the evaluated programs with SpecFuzz and \toolname{}-SpecFuzz.}{
  \rowcolors{3}{gray90}{}
  \resizebox{0.45\textwidth}{!}{
    {\renewcommand{\arraystretch}{1.3}
    \begin{tabular}{c<{\hspace{1pc}} c<{\hspace{1pc}}c c} %
      \toprule
      \multirow{2}{*}{Program} & \multirow{2}{*}{SpecFuzz} & \multicolumn{2}{c}{\toolname{}-SpecFuzz} \\
      & & \normalfnname{} & \specfnname{} \\
      \midrule
      libyaml & 70.82\% & 75.77\% & 72.78\% \\
      libhtp & 64.52\% & 64.88\% & 57.19\% \\
      brotli & 69.03\% & 80.64\% & 81.76\% \\
      openssl & 23.35\% & 24.98\% & 21.03\% \\
      \bottomrule
    \end{tabular}}\label{tab:expsf-cov}
  }
}
\end{table}

\begin{table}[t]
  \centering
  \caption{Number of gadgets found from the evaluated programs with SpecFuzz and \toolname{}-SpecFuzz.}{
  \rowcolors{1}{}{gray90}
  \resizebox{0.45\textwidth}{!}{
    {\renewcommand{\arraystretch}{1.3}
    \begin{tabular}{c<{\hspace{1pc}} c<{\hspace{1pc}}c} %
      \toprule
      Program & SpecFuzz Gadgets & \toolname{}-SpecFuzz Gadgets \\
      \midrule
      libyaml & 47 & \textbf{323} \\
      libhtp & 347 & \textbf{355} \\
      brotli & 108 & \textbf{124} \\
      openssl & 785 & \textbf{814} \\
      \bottomrule
    \end{tabular}}\label{tab:expsf-gadget}
  }
}
\end{table}

We evaluate the gadget detectability of \toolname{}-SpecFuzz in real-world binary applications by fuzzing them for 24 hours.
Note that these experiments are executed only with 4 threads (as opposed to 8 in \cref{ssec:exp-fuzz-v2,ssec:exp-fuzz-v1}), and nested speculation support is disabled.
We collect the number of AddressSanitizer violations (SpecFuzz-policy gadgets) in speculation simulation and the final reached code coverage in both the \normalfnname{} and \specfnname{} following the policy described above.
We do not discuss the actual exploitability (false positives) in this experiment. 
For coverage comparison, SpecFuzz shares the same normal coverage tracing mechanism with \toolname{}-SpecFuzz, so they are directly comparable.
Unfortunately, SpecFuzz does not collect speculative coverage, so a comparison could not be made.

\cref{tab:expsf-cov} shows the maximum reached coverage of each program.
\toolname{}-SpecFuzz outperforms SpecFuzz on the final normal coverage of all tested programs, which can likely be attributed to the much lower run-time overhead, leading to increased fuzzing throughput.

Next, the number of gadgets found is shown in \cref{tab:expsf-gadget}.
While general beliefs on compiler-based vs. binary-based analysis seem to suggest that \toolname{}-SpecFuzz shall detect slightly fewer gadgets than compiler-based instrumentation due to the lower object protection granularity on the stack and the inability to detect global object overflows, the result shows otherwise: on all evaluated programs, \toolname{}-SpecFuzz outperforms SpecFuzz in gadget detectability.
Although the coverage advantage of \toolname{}-SpecFuzz certainly plays a role, coverage alone does not explain the extreme magnitude of gadget count difference observed in \texttt{libyaml}.

In search of an explanation, we examined the implementation of SpecFuzz.
We find the root cause of the problem originates from SpecFuzz's ASan instrumentation, which is handled by LLVM and at an earlier stage before other SpecFuzz instrumentation passes.
This generates two issues: (1) SpecFuzz cannot distinguish the instructions that are part of the original program logic and that are inserted by ASan, and therefore tends to execute less code before reaching the rollback limit (as discussed in \cref{ssec:motivations-compiler}).
(2) The compiler makes varied optimization choices with the initial presence of ASan, resulting in different program behaviors on the binary level.
In practice, we find that (2) explains the majority of SpecFuzz's false negatives in \texttt{libyaml} (we examine one such example in detail in \cref{ssec:apdx-case-study-sf}).

Although the above conclusion seems to suggest that SpecFuzz's implementation choices have been the main limiting factor here, we consider that all analysis tools that rely on compiler-frontend passes would likely be subject to similar issues (thus, including Kasper\cite{Kasper}).
Such problems can be avoided with binary-based analysis or compiler-based analysis passes that are purely implemented in the backend.

\subsection{Case study: speculative stack underflow in libyaml}\label[appendix]{ssec:apdx-case-study-sf}

\begin{lstlisting}[style=my-lst-style-linenum, float=t, caption={A speculative stack underflow in libyaml that is missed by SpecFuzz.}, label={lst:case-study-sf}]
static int
yaml_parser_parse_block_sequence_entry(
  /* ... */, int first) { // first == true
  yaml_token_t *token;

  // first == true -> stack is empty
@\lstcolourline{yellow!15}@  if (first) { // mispredicted as false
@\lstcolourline{gray!30}@    // will not execute
@\lstcolourline{gray!30}@    token = PEEK_TOKEN(parser);
@\lstcolourline{gray!30}@    if (!PUSH(token->start_mark))
@\lstcolourline{gray!30}@      return 0;
@\lstcolourline{gray!30}@    SKIP_TOKEN(parser);
  }

@\lstcolourline{yellow!15}@  // next token read is misaligned
@\lstcolourline{yellow!15}@  token = PEEK_TOKEN(parser);
  if (!token) return 0;

  if (token->type == ENTRY_TOKEN)
    // ...
  else if (token->type == END_TOKEN)
    // ...
  else {
@\lstcolourline{red!15}@    // underflow because stack is still empty
@\lstcolourline{red!15}@    return error(POP());
  }
}
\end{lstlisting}

\begin{lstlisting}[style=my-lst-style-linenum, float=t, caption={Disassembly of the \texttt{POP} operation.}, label={lst:case-study-sf-disasm}, language={[x64]Assembler}]
; Without Instrumentation
movups xmm0, xmmword ptr [rcx - 24]
movaps xmmword ptr [rsp + 32], xmm0
mov rax, qword ptr [rcx - 8]
mov qword ptr [rsp + 48], rax

; With Compiler Asan
call __asan_memcpy
\end{lstlisting}

We detected a speculative stack underflow vulnerability in \texttt{libyaml} with \toolname{}-SpecFuzz, which was missed by SpecFuzz.
\cref{lst:case-study-sf} shows the code snippet that contains the vulnerability.
A stack maintains the tokens and is empty at first.
When \texttt{first} is true (line~7), the function peeks the next token and pushes it onto the stack (line~9).
However, if the branch is mispredicted and the \texttt{if} block is not executed, the stack remains empty, and the next token read in the immediately succeeding statement is misaligned (line~16), and the function falls into the error branch (line~23).
In the error branch, it attempts to pop a token that was never pushed onto the stack because of the branch misprediction, triggering the speculative stack overflow (line~25).

This gadget is unlikely to be exploitable in practice (and thus not reported by \toolname{} with Kasper policy) for the following reasons.
(1) The argument \texttt{first} is passed by register in the x86-64 System V calling convention, so the branch resolves quickly.
(2) The out-of-bounds access only allows off-by-one underflow and is unlikely to leak secrets.
Nevertheless, it matches the definition of gadgets in the SpecFuzz policy.

\textbf{Challenges in detecting this vulnerability.}
This gadget remains undetected by the original SpecFuzz.
To investigate this, we disassemble the instrumented program, shown in \cref{lst:case-study-sf-disasm}.
The stack maintains elements that are 24 bytes each, so the memory transfers such as the \texttt{PUSH} and \texttt{POP} are generated as the combination of two SSE move instructions \texttt{movups}/\texttt{movaps} and two \texttt{mov}s.
However, SpecFuzz requires the instrumentation of the program with compiler-based ASan, and such memory transfers tend to be compiled into \texttt{\_\_asan\_memcpy} calls instead.
The external call to \texttt{\_\_asan\_memcpy} triggers an unconditional rollback so the gadget remains undetectable.
In contrast, \toolname{} does not suffer from such inaccuracies as it directly instruments the binary. \looseness=-1


==> figs/expsf-runtime-overhead.tex <==
\begin{figure}[t]
\begin{tikzpicture}%

\begin{axis}[
name=overheadfig,
axis x line*=bottom, y axis line style={draw=none},
ymajorgrids=true, yminorgrids=true, minor tick num=1,
major grid style={line width=.6pt,draw=gray!60},
ybar=0pt, bar width=.5cm, xtick=data, ymin=0, ymax=601,
width=0.48\textwidth, height=4cm,
ylabel={Normalized Run Time},
yticklabel={\pgfmathprintnumber{\tick}x},
symbolic x coords={libyaml, libhtp, brotli, openssl},
xtick style={draw=none}, x axis line style={line width=1pt,draw=black},
enlarge x limits=0.13,
legend style={at={(1, 1)}, anchor=north east, font=\footnotesize},
legend image code/.code={\draw [#1] (0cm,-0.1cm) rectangle (0.2cm,0.15cm); },
legend cell align={left},
legend to name=overheadlegend_expsf_runtime, 
legend columns=-1
]
\addplot[fill=black!85]
coordinates {
    (libyaml, 590)
    (libhtp, 124)
    (brotli, 487)
    (openssl, 298)
};

\addplot[fill=black!55]
coordinates {
    (libyaml, 222)
    (libhtp, 54)
    (brotli, 149)
    (openssl, 135)
};


\legend{SpecFuzz, \toolname{}-SpecFuzz}
\end{axis}

\node () at (overheadfig.north) [above, yshift=.3cm, text=black] {\nocolorref{overheadlegend_expsf_runtime}};

\end{tikzpicture}
\caption{Execution time of the instrumented programs with large crafted inputs, normalized to the execution time of the native versions. Lower is better. Averaged over 10 runs.}
\label{fig:expsf-runtime-overhead}
\end{figure}


==> snippets/acm-copyright.tex <==
\author{Fangzheng Lin}
\email{lin.f.f849@m.isct.ac.jp}
\affiliation{
  \institution{Institute of Science Tokyo}
  \state{Tokyo}
  \country{Japan}
}

\author{Zhongfa Wang}
\email{wang.z.e488@m.isct.ac.jp}
\affiliation{
  \institution{Institute of Science Tokyo}
  \state{Tokyo}
  \country{Japan}
}

\author{Hiroshi Sasaki}
\email{sasaki@ict.eng.isct.ac.jp}
\affiliation{
  \institution{Institute of Science Tokyo}
  \state{Tokyo}
  \country{Japan}
}

\copyrightyear{2025}
\acmYear{2025}
\setcopyright{cc}
\setcctype{by}
\acmConference[CGO '25]{Proceedings of the 23rd ACM/IEEE International Symposium on Code Generation and Optimization}{March 01--05, 2025}{Las Vegas, NV, USA}
\acmBooktitle{Proceedings of the 23rd ACM/IEEE International Symposium on Code Generation and Optimization (CGO '25), March 01--05, 2025, Las Vegas, NV, USA}
\acmDOI{10.1145/3696443.3708936}
\acmISBN{979-8-4007-1275-3/25/03}

\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10002978.10003006.10011634.10011635</concept_id>
<concept_desc>Security and privacy~Vulnerability scanners</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10002978.10003001.10010777.10011702</concept_id>
<concept_desc>Security and privacy~Side-channel analysis and countermeasures</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10011007.10011006.10011041.10011046</concept_id>
<concept_desc>Software and its engineering~Translator writing systems and compiler generators</concept_desc>
<concept_significance>300</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Security and privacy~Vulnerability scanners}
\ccsdesc[300]{Security and privacy~Side-channel analysis and countermeasures}
\ccsdesc[300]{Software and its engineering~Translator writing systems and compiler generators}

\keywords{Spectre gadget detector, binary instrumentation}



==> snippets/lstlinebgrd-workaround.tex <==
\makeatletter
\let\old@lstKV@SwitchCases\lstKV@SwitchCases
\def\lstKV@SwitchCases#1#2#3{}
\makeatother
\usepackage{lstlinebgrd}
\makeatletter
\let\lstKV@SwitchCases\old@lstKV@SwitchCases

\lst@Key{numbers}{none}{%
    \def\lst@PlaceNumber{\lst@linebgrd}%
    \lstKV@SwitchCases{#1}%
    {none:\\%
     left:\def\lst@PlaceNumber{\llap{\normalfont
                \lst@numberstyle{\thelstnumber}\kern\lst@numbersep}\lst@linebgrd}\\%
     right:\def\lst@PlaceNumber{\rlap{\normalfont
                \kern\linewidth \kern\lst@numbersep
                \lst@numberstyle{\thelstnumber}}\lst@linebgrd}%
    }{\PackageError{Listings}{Numbers #1 unknown}\@ehc}}
\makeatother

